ConTesse: Accurate Occluding Contours for Subdivision Surfaces

This paper proposes a method for computing the visible occluding contours of subdivision surfaces. The paper first introduces new theory for contour visibility of smooth surfaces. Necessary and sufficient conditions are introduced for when a sampled occluding contour is valid, that is, when it may be assigned consistent visibility. Previous methods do not guarantee these conditions, which helps explain why smooth contour visibility has been such a challenging problem in the past. The paper then proposes an algorithm that, given a subdivision surface, finds sampled contours satisfying these conditions, and then generates a new triangle mesh matching the given occluding contours. The contours of the output triangle mesh may then be rendered with standard non-photorealistic rendering algorithms, using the mesh for visibility computation. The method can be applied to any triangle mesh, by treating it as the base mesh of a subdivision surface.

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/bhk2014.tex <==
\newcommand{\bhkwidth}{1.5in}%
\begin{figure*}
    \centering
    \begin{tabular}{ccc}
    \includegraphics[width=\bhkwidth]{comparison/killeroo_2014a.pdf}~~
&        \includegraphics[width=2in]{comparison/killeroo_2014c.pdf}
&        \includegraphics[width=\bhkwidth]{comparison/killeroo_cam212_2014_inconsist12.jpg} \\
(a) $1\times$/$40\times$ & (b) $1600\times$ & (c) Mesh side view
\end{tabular}
        \caption{Invalid contours with \cite{Benard:2014}.
        (a)
        B\'{e}nard et al.~produce highly refined contours using root-finding. Nonetheless, the contours may fail to be WSO. In the example here, a twist occurs in the sampling near a cusp, similar to the example in Figure \ref{fig:invalid}(b). 
        (b)
        In image-space, this twist is an \textit{extremely} thin structure, nearly invisible even at the $1600\times$ zoom shown here.
        (c) As a result, B\'{e}nard et al.'s triangulation produces an inconsistent triangle in this region, shown in a side view highlighted in purple.  This instance is occluded and thus does not affect visibility, but there is no guarantee that this will always be the case.
        For this example, the output includes 11 inconsistent triangles out of 546,624 that were generated. 
        Our method produces 100\% consistent triangles, generating only 55,476 triangles for this view (Figure \ref{fig:results}), and performing substantially faster (2 minutes for our method, and 10 minutes for B\'{e}nard et al.)
        (Killeroo
\copyright\ headus.com.au)  
    \label{fig:bhk2014}}
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/invalid.tex <==
\begin{figure*}
    \centering
    (a)
            \includegraphics[width=1in]{invalid/invalid-smooth.pdf}
                \includegraphics[width=1in]{invalid/invalid-smooth-triangulated.pdf}
                \includegraphics[width=1in]{invalid/valid-smooth-triangulated.pdf}
(b) \includegraphics[width=1.5in]{invalid/skinny_cusp.pdf} 
\includegraphics[width=1.5in]{invalid/cusp_sampling.pdf}

    \caption{Invalid curves. (a) An example in which sparsely-sampled points around a simple smooth curve produce an invalid 2D polygon (in grey). The polygon self-intersects, and cannot be triangulated without introducing a twist in the resulting 3D surface. In this case, adding a sample point (purple) makes the polygon valid.
    (b) A common case where the polygon is very skinny near a cusp, and undersampling introduces a loop near the cusp.
    }
    \label{fig:invalid}
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/ocg.tex <==
\newcommand{\pswidth}{1.5in}
\begin{figure}
    \centering
    (a)
    \includegraphics[width=0.43\linewidth]{definitions/torus-mesh.pdf}
    ~%
    (b)
    \includegraphics[width=0.43\linewidth]{definitions/torus-smooth.pdf}
    \caption{Definition of occluding contour (or apparent contour) and occluding contour generator, for meshes (a) and smooth surfaces (b), from \bh{3.4,7.2}. The occluding contour describes occlusion boundaries in the image.
    Throughout the paper, we use the follow color scheme: 
    contour points are \textcolor{red}{\bf red}, front-facing points are \textcolor{Orange}{\bf yellow}, and back-facing points are \textcolor{Blue}{\bf blue}.
    }
    \label{fig:ocg}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/overview.tex <==
\begin{figure*}
\centering
\includegraphics[width=7in]{overview3.pdf}
\caption{Overview of the ConTesse algorithm. The input is a smooth surface viewed from a camera center \textbf{c}. An initial triangle mesh is computed, with contour edges inserted by root-finding. The contours partition the object into WSOH regions. Each region is decomposed into simple polygons, using cuts to remove holes and WSO triangulation to decompose self-overlapping regions. Each simple polygon is then triangulated and lifted to 3D, and these triangulations are stitched to produce the output mesh. This mesh can then be used as input to conventional non-photorealistic rendering algorithms.
\label{fig:contesse-overview}}
\end{figure*}


==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/plots.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=3.3in]{plots/computation_time_plot_ff.pdf}
    \includegraphics[width=3.3in]{plots/output_size_plot_ff.pdf}    
    \caption{Computation time and output size for each of the inputs. These results are for generating front-faces only; output triangles for back-facing regions are not generated in these plots, since they would almost never be used in practice.
    Each dot represents one or more of the 1580 test cases (mesh, camera), with the number of subdivision rounds required for that case color-coded. The vertical strip of dots at 39,576 input triangles are different tests on the Angela mesh.
    The green diagonal line shows where unity values would occur on the plot (i.e., one input for one output).
    These computations were performed on a MacBook Pro M1, 3.2Ghz, 16Gb memory.
    }
        \label{fig:plots}
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/problem_convex.tex <==

\begin{figure}
    \centering
    (a)
\includegraphics[width=1.5in]{convex/convex-smooth2.pdf}%
~%
(b)
\includegraphics[width=1.5in]{convex/convex-mesh3.pdf} 
    \caption{Convex contour tessellation.  
    (a) The input is a convex smooth surface viewed from a camera position $\bc$. The contour projects to a simple convex curve.
     (b)
    Naively converting the smooth surface to a triangle mesh produces a mesh for which the occluding contour projects to a curve with very different topology. The new topology can be  badly behaved, leading to many visibility errors  \cite{Benard:2014}. 
     }
    \label{fig:problem}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/region_types.tex <==
\begin{figure*}
    \centering
\begin{tabular}{cccc}
\multicolumn{4}{c}{\Large (a) \textbf{Simple}} \\
    \includegraphics[height=1in]{polygon_types/convex_front.pdf} &
    \includegraphics[height=1in]{polygon_types/convex_side.pdf} &
    \includegraphics[height=1in]{polygon_types/convex_polygon.pdf} &
    \includegraphics[height=1in]{polygon_types/convex_polygon.pdf} \\
    Camera view &
    Side view &
    2D polygon &
    2D embedding of polygon \\
    of 3D shape &
    &
    from points sampled on contour &
    for visualization
\\
        \hline\\
\multicolumn{4}{c}{(b) \Large \textbf{Self-Overlapping}} \\
    \includegraphics[height=1in]{polygon_types/so_front.pdf} &
    \includegraphics[height=1in]{polygon_types/so_side.pdf} &
    \includegraphics[height=1in]{polygon_types/so_polygon.pdf} &
    \includegraphics[height=1in]{polygon_types/so_immersion.pdf} \\
    Camera view &
    Side view &
    2D polygon &
    2D embedding of polygon
\\
        \hline\\
    \multicolumn{4}{c}{\Large (c) \textbf{Weakly Self-Overlapping (WSO)}} \\
\includegraphics[height=1in]{polygon_types/wso_front.pdf} &
    \includegraphics[height=1in]{polygon_types/wso_side.pdf}  &
    \includegraphics[height=1in]{polygon_types/wso_polygon.pdf} & 
    \includegraphics[height=1in]{polygon_types/wso_immersion2.pdf} \\ 
    Camera view &
    Side view &
    2D polygon &
    2D embedding of polygon
\\
            \hline\\
    \multicolumn{4}{c}
{\Large (d) \textbf{Weakly Self-Overlapping with Holes (WSOH)}} \\
    \includegraphics[height=1in]{polygon_types/wsoh_front.pdf} &
    \includegraphics[height=1in]{polygon_types/wsoh_side.pdf} &
    \includegraphics[height=1in]{polygon_types/wsoh_polygon.pdf} &
    \includegraphics[height=1in]{polygon_types/wsoh_immersion.pdf} \\
    Camera view &
    Side view &
    2D region &
    2D embedding of region
    \end{tabular}
    \caption{The four categories of contour regions in 3D, and how they project to 2D. Each row shows a smooth surface from the camera view and from a side view (first and second columns) with the contour in \textbf{\textcolor{red}{red}}, the front-facing region in \textcolor{Orange}{\bf yellow}, back-facing regions in \textcolor{Blue}{\bf blue}, and cusps/singularities as red dots.
    A 2D projection of the front-facing region is shown (third column), with vertices sampled from the contour. The final column is meant to aid in understanding the 2D region; vertices are translated to unfold the region.
    \label{fig:region_types}}
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/results.tex <==
\newcommand{\figwidth}{1.6in}
\newcommand{\figheight}{1in}
\begin{figure*}
\centering
\begin{tabular}{cccc}
(a) Camera view & (b) Side view & (c) Output curve network & (d) Occluding contours \\
\includegraphics[width=\figwidth]{results/spot_control_mesh_cam212_contour.jpg} &
\includegraphics[width=\figwidth]{results/spot_control_mesh_cam212_side.jpg} & 
\includegraphics[width=\figwidth]{results/spot_control_mesh_cam212_highlight.pdf} &
\includegraphics[width=\figwidth]{results/spot_control_mesh_cam212_qi_chained.pdf} \\

\includegraphics[width=\figwidth]{results/torus_quad_v1_cam222_contour.jpg} &
\includegraphics[width=\figwidth]{results/torus_quad_v1_cam222_side.jpg} &
\includegraphics[width=\figwidth]{results/torus_quad_v1_cam222_highlight.pdf} &
\includegraphics[width=\figwidth]{results/torus_quad_v1_cam222_highlight_black.pdf} \\





\includegraphics[width=\figheight]{results/bunny_000001_contour.jpg} &
\includegraphics[width=\figheight]{results/bunny_000001_side.jpg} &
\includegraphics[width=\figheight]{results/bunny_000001_highlight.pdf} &
\includegraphics[width=\figheight]{results/bunny_000001_qi_chained.pdf} \\


\includegraphics[width=\figwidth]{results/killeroo_small_cam212_contour.jpg} &
\includegraphics[width=\figheight]{results/killeroo_small_cam212_side.jpg} &
\includegraphics[width=\figwidth]{results/killeroo_small_cam212_highlight.pdf} &
\includegraphics[width=\figwidth]{results/killeroo_small_cam212_qi_chained.pdf} \\


\end{tabular}
\caption{
Examples of the ConTesse algorithm applied to various surfaces and camera views. Each example is a commonly-used mesh in geometry processing, treated as a Catmull-Clark base mesh. (a) Camera view of the output mesh, (b) side view of the output mesh, (c) view graph (curve network) of the visible occluding contours of the output mesh, with cusps marked in orange and 2D intersections in green, and
(d) occluding contours, after computing visibility.
(Public domain Spot model by Keenan Crane, Killeroo \copyright\ headus.com.au.)
\label{fig:results}
}
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/singularity.tex <==
\newcommand{\singwdth}{0.9in}

\begin{figure}
    \centering
    (a)
    \includegraphics[width=\singwdth]{singularity/sing2.pdf}
\hfill
(b)
    \includegraphics[width=\singwdth]{singularity/sing4.pdf}
    \hfill
    (c)
    \includegraphics[width=\singwdth]{singularity/sing3.pdf}
    \caption{Singularity side determination. (a) At a cusp, one of the two adjacent regions self-overlaps in image-space, i.e., the total rotation angle of the polygons $\Theta>2\pi$.
    (b) In the tangent plane of a cusp on a smooth surface, the curve Laplacian points toward the smaller, non-overlapping region, which is back-facing (blue) in this example.
    (c) Since we are operating with a discrete mesh output, we compute the discrete curve Laplacian, and tag a singularity in the region (yellow) that it does not point to.
    \label{fig:singularity-direction}}
\end{figure}


==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/smooth_tangents.tex <==
\begin{figure}
    \centering
    \includegraphics[width=2.5in]{smooth_tangents.pdf}
    \caption{Elements of the proof of Theorem \ref{thm:wso_smooth}. See text for details.}
    \label{fig:smooth_tangents}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/spiral.tex <==
\begin{figure}
    \centering
    (a)
    \includegraphics[width=1in]{vertex_theta.pdf}
    (b)
    \includegraphics[width=1in]{vertex_spiral.pdf}
    \caption{Rotations around a vertex in 2D. Let $\Theta$ be the sum of the angles adjacent to a vertex.
    (a) 
    Normally, at interior vertices of a typical planar triangulation with positive orientation, there are no overlaps or folds, implying $\Theta=2\pi$.
    (b) A vertex where $\Theta=4\pi$. We disallow this case in the WSOH definition.
    \label{fig:spiral} }
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/steps_convex.tex <==
\begin{figure}
    \centering
        
    \includegraphics{convex/convex_steps2.pdf} 
        
    \caption{Steps of the convex surface tessellation algorithm. 
    (a) Points are sampled along the smooth surface contour. These points are projected to a 2D polygon in image space.
    (b) The polygon is triangulated in image space.
    (c) 2D triangles are lifted to 3D, by projecting their vertices back onto the original surface, in both the front-facing and back-facing regions. 
    }
    \label{fig:steps}
\end{figure}




==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/stylized_results.tex <==
\newcommand{\sfigwidth}{1.5in}
\newcommand{\sfigheight}{1.5in}

\begin{figure*}
\includegraphics[height=1.5in]{results/spot_cam212_topo_dots.jpg}
\includegraphics[width=2in]{results/torus_quad_v1_cam222_topo_scribble.jpg} 
\includegraphics[height=1.5in]{results/bunny_000001_loop_qi_chained.jpg} 
\includegraphics[height=1.5in]{results/killeroo_small_cam212_topo_wedge.jpg}  \\
\includegraphics[height=\sfigheight]{more_results/bigguy_cam112_side.jpg}
\includegraphics[height=\sfigheight]{more_results/bigguy_cam112_qi_chained_candle.jpg}
\includegraphics[height=\sfigheight]{more_results/BSoD-ItCA-final_000004_side.jpg}
\includegraphics[height=\sfigheight]{more_results/BSoD-ItCA-final_000004_scribble_qi_chained.jpg} \includegraphics[height=\sfigheight]{more_results/ogre_controlmesh_cam222_side.jpg}
\includegraphics[height=\sfigheight]{more_results/ogre_controlmesh_cam222_qi_chained_scribble.jpg} \\
\includegraphics[height=\sfigheight]{more_results/monsterfrog_cam212_side.jpg}
\includegraphics[height=\sfigheight]{more_results/monsterfrog_cam212_qi_chained_candle.jpg} 
\includegraphics[height=\sfigheight]{more_results/pig_quad_controlmesh_cam222_side_rotated.jpg}
\includegraphics[height=\sfigheight]{more_results/pig_quad_controlmesh_cam222_qi_chained_candle_rotated.jpg}
\caption{Stylized versions of the contours from Figure \ref{fig:results}, and results from three more models in our dataset. Note that we do not render mesh self-intersections. 
(Public domain Pig, ogre, and Spot models by Keenan Crane,
Killeroo \copyright\ headus.com.au,
Bigguy and Monster Frog \copyright\ Bay Raitt, Walking Man \copyright\ Ryan Dale.)
\label{fig:stylized_results}} 
\end{figure*}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/subdivided_results.tex <==
\begin{figure}
\centering
\includegraphics[width=1.5in]{results/subdivided/torus_quad_v1_cam222_contour.jpg}
\includegraphics[width=1.5in]{results/subdivided/torus_quad_v1_cam222_side_highpoly.jpg}
\caption{Finer-resolution meshes may be obtained by increasing the number of initial subdivision levels. Here the torus was subdivided twice initially, as compared to once in Figure \ref{fig:results}.
\label{fig:subdivided_results}
}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/table_stats.tex <==
\begin{table*}[t]
\centering
    \begin{tabular}{|lcc|ccc|ccc|}
      \hline
      &&&\multicolumn{3}{c|}{\bf B\'{e}nard et al.~\shortcite{Benard:2014}} &
      \multicolumn{3}{c|}{\bf Our method} \\ \hline
      \multirow{2}{*}{Sequence} & Input & \multirow{2}{*}{Frames} &
      Output & Inconsistent & Time &
      Output & Inconsistent & Time 
      \\
      &faces&&faces&faces&(sec.)&faces&faces&(sec.)\\
      \hline
      Stanford Bunny & 42,928 & 400 &
      \quad $51,336 \pm 1,383$ & $7.6 \pm 4.4$ & $120 \pm35$ &
      $23,424 \pm518.1$ & 0 & $12 \pm2.2$\\
      Angela's face & 39,576 & 150 &
      \, $50,907 \pm693$ & $14 \pm4.4$& $170 \pm42$ &
      $26,642 \pm6,286$ & 0 & $28 \pm22$ \\
      Walking Man & 30,912 & 120 &
      $158,184 \pm663$ & $2.3 \pm2.1$ & $160 \pm15$ &
      $10,825 \pm2,620$ & 0  & $12 \pm10$\\
      \hline
    \end{tabular}
\caption{Statistics of our mesh generation algorithm on three of the animation sequences tested by \cite{Benard:2014}. The ``Red'' animation is omitted because it is proprietary.
The numbers are averaged over animation frames, which we list together with the standard deviation in each case. 
Our method produces no inconsistencies, far fewer output faces (roughly half), and runs much faster ($6\times$ to $13\times$ speedup). These values are for generating front and back faces, though back-faces would almost never be generated in practice.  Details: Both methods were run with a single thread on the same MacBook Pro (3.1GHz Intel Core i5 CPU, 8GB of memory).  The number of input faces is after one round of subdivision, and computation times are for mesh generation only, not stylization. We report fewer input faces for ``Walking Man'' because our method using 1 subdivision level as the minimum subdivision level, rather than 2 subdivisions used by B\'enard et al.}
\label{table:benard}
\end{table*}



==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/teaser1.tex <==
\newcommand{\tfigwidth}{1.5in}
\newcommand{\tfigheight}{.75in}

\begin{teaserfigure}
\centering
\begin{tabular}{c@{}c@{}c@{}c}
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_input_smooth.jpg} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_contour.jpg}%
\includegraphics[width=\tfigheight]{results/fertility_cam120_side.jpg}  &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_highlight.pdf} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_topo_loop.jpg} \\
(a) & (b) & (c) & (d)
\end{tabular}
    \caption{Given (a) a smooth 3D surface $\cS$ and a camera viewpoint, our method produces (b) a triangle mesh $\cM$ where the occluding contour of the mesh accurately approximates the occluding contour of the smooth surface. Standard algorithms may then be used to extract (c) the view map of occluding contours, and to (d) stylize them.
    (Fertility courtesy UU from AIM@SHAPE-VISIONAIR Shape Repository).
    }
    \label{fig:teaser}
\end{teaserfigure}


==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/teaser_arxiv.tex <==
\newcommand{\tfigwidth}{1.5in}
\newcommand{\tfigheight}{.75in}

\begin{figure*}
\centering
\begin{tabular}{c@{}c@{}c@{}c}
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_input_smooth.jpg} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_contour.jpg}%
\includegraphics[width=\tfigheight]{results/fertility_cam120_side.jpg}  &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_highlight.pdf} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_topo_loop.jpg} \\
(a) & (b) & (c) & (d)
\end{tabular}
    \caption{Given (a) a smooth 3D surface $\cS$ and a camera viewpoint, our method produces (b) a triangle mesh $\cM$ where the occluding contour of the mesh accurately approximates the occluding contour of the smooth surface. Standard algorithms may then be used to extract (c) the view map of occluding contours, and to (d) stylize them.
    }
    \label{fig:teaser}
\end{figure*}


==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/trivial.tex <==
\begin{figure}
    \centering
\includegraphics[width=1.5in]{results/fertility_rotate/fertility_cam120_qi_trivial_thicker.pdf}
    \caption{
    Naive visibility. In this example, the occluding contour has been sampled into line segments, and then visibility for each segment was computed by a separate ray test against a dense triangulation of the surface. This naive strategy produces unreliable visibility, such as incorrect gaps in the contours. Most algorithms use a combination of heuristics that can greatly improve over a naive result, but they cannot remove all visibility errors.
(Fertility by UU from AIM@SHAPE-VISIONAIR Shape Repository).    }
    \label{fig:trivial}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/twist_cases.tex <==
\begin{figure}
\centering
Case 1, Tiny hole:\\
\includegraphics[width=3in]{twists/smallhole2.pdf}\\
Case 2, Inverted fishtail:\\
\includegraphics[width=3in]{twists/invertedfishtail2.pdf}\\
Case 3, Twisted cusp: \\
\includegraphics[width=3in]{twists/cusp.pdf}\\
Case 4, Twisted tube:\\
\includegraphics[width=3in]{twists/skinny.pdf}\\
Case 5, Outside cusp:\\
\includegraphics[width=3in]{twists/cusphole2.pdf}
\caption{The five cases of twists that we detect and resolve; see text for details.
\label{fig:twist_cases}
}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/wso_def.tex <==
\begin{figure}
    \centering
    (a)\includegraphics[width=3in]{wso_def.pdf}
    (b)\includegraphics[width=3in]{figures_reduced/wsoh_def.pdf}
\caption{(a) Elements of the definition of Weakly Self-Overlapping (WSO), shown here with a self-overlapping polygon $P$. There exists a mesh $M$ with disk topology and a map $f$ such that $P$ is the boundary of $f(M)$, and the mapping $f(M)$ has no flipped triangles or spiral structures.
    (b) Elements of the WSOH definition.  A set of polygons $\cP=\{P_1,P_2\}$ form the boundary of a mapping $f(M)$, where $M$ is a mesh with holes. Some vertices are numbered to show the correspondence.
    (Figure (a) from \cite{WeberZorin}, used courtesy the authors.)
    }
    \label{fig:wso_def}
\end{figure}

==> ConTesse_ Accurate Smooth Occluding Contours_arXiv/figure_tex/yeahright.tex <==
\newcommand{\yrheight}{4in}

\begin{figure*}
    \centering
    \includegraphics[height=\yrheight]{results/yeahright_220.pdf}
        \includegraphics[height=\yrheight]{results/yeahright_100_zoom.pdf}
\caption{Two views of the complex ``Yeah, Right'' model, which has genus 131. (Public domain model by Keenan Crane.)}
    \label{fig:yeahright}
\end{figure*}

\begin{figure}
\centering
\includegraphics[width=3in]{results/yeah_cam220_side.jpg}
\caption{Side view of the output triangulation of ``Yeah, Right,'' for the leftmost rendering in Figure \ref{fig:yeahright}}
\label{fig:yeahrightside}
\end{figure} 

==> figure_tex/teaser_arxiv.tex <==
\newcommand{\tfigwidth}{1.5in}
\newcommand{\tfigheight}{.75in}

\begin{figure*}
\centering
\begin{tabular}{c@{}c@{}c@{}c}
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_input_smooth.jpg} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_contour.jpg}%
\includegraphics[width=\tfigheight]{results/fertility_cam120_side.jpg}  &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_highlight.pdf} &
\includegraphics[width=\tfigwidth]{results/fertility_rotate/fertility_cam120_topo_loop.jpg} \\
(a) & (b) & (c) & (d)
\end{tabular}
    \caption{Given (a) a smooth 3D surface $\cS$ and a camera viewpoint, our method produces (b) a triangle mesh $\cM$ where the occluding contour of the mesh accurately approximates the occluding contour of the smooth surface. Standard algorithms may then be used to extract (c) the view map of occluding contours, and to (d) stylize them.
    }
    \label{fig:teaser}
\end{figure*}

